Ghost in the Minecraft: Generally Capable Agents for Open-World Environments via Large Language Models with Text-based Knowledge and Memory

The captivating realm of Minecraft has attracted substantial research interest in recent years, serving as a rich platform for developing intelligent agents capable of functioning in open-world environments. However, the current research landscape predominantly focuses on specific objectives, such as the popular "ObtainDiamond" task, and has not yet shown effective generalization to a broader spectrum of tasks. Furthermore, the current leading success rate for the "ObtainDiamond" task stands at around 20%, highlighting the limitations of Reinforcement Learning (RL) based controllers used in existing methods. To tackle these challenges, we introduce Ghost in the Minecraft (GITM), a novel framework integrates Large Language Models (LLMs) with text-based knowledge and memory, aiming to create Generally Capable Agents (GCAs) in Minecraft. These agents, equipped with the logic and common sense capabilities of LLMs, can skillfully navigate complex, sparse-reward environments with text-based interactions. We develop a set of structured actions and leverage LLMs to generate action plans for the agents to execute. The resulting LLM-based agent markedly surpasses previous methods, achieving a remarkable improvement of +47.5% in success rate on the "ObtainDiamond" task, demonstrating superior robustness compared to traditional RL-based controllers. Notably, our agent is the first to procure all items in the Minecraft Overworld technology tree, demonstrating its extensive capabilities. GITM does not need any GPU for training, but a single CPU node with 32 CPU cores is enough. This research shows the potential of LLMs in developing capable agents for handling long-horizon, complex tasks and adapting to uncertainties in open-world environments. See the project website at https://github.com/OpenGVLab/GITM.

==> tables/ablation-memory.tex <==
\setlength{\tabcolsep}{6pt}
\begin{table}
    \centering
    \begin{tabular}{lccc}
    \toprule
    Memory Content & \makecell{Number of\\ Queries} & \makecell{Number of\\Actions} & \makecell{Number of\\Steps} \\
    \midrule
    Wooden pickaxe & & & \\
    Stone pickaxe & & & \\
    Iron pickaxe & & & \\
    Diamond & & & \\
    \bottomrule
    \end{tabular}
    \caption{Memory learning process. (can be a figure)}
    \label{tab:ablation_memory}
\end{table}

==> tables/ablation-sub-goal_parsing.tex <==
\setlength{\tabcolsep}{6pt}
\begin{table}
    \centering
    \begin{tabular}{l|ccccc}
    \toprule
    Success Rate & \makecell{Crafting\\Table} & \makecell{Wooden\\Pickaxe} & \makecell{Stone\\Pickaxe} & \makecell{Iron\\Pickaxe} & Diamond \\
    \midrule
    w/o sub-goal & & & \\
    w/ sub-goal & & & \\
    \bottomrule
    \end{tabular}
    \caption{Ablation of sub-goal parsing.}
    \label{tab:ablation_decompose}
\end{table}

==> tables/exp-comparison.tex <==
\setlength{\tabcolsep}{5pt}
\setlength{\doublerulesep}{2\arrayrulewidth}
\begin{table}[t]
    \centering
    \small
    \caption{Comparison of our GMIT with previous methods on the \texttt{ObtainDiamond} challenge.}
    \begin{tabular}{l|ccccc}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{5}{c}{Success Rate (\%)}\\
    & \mccraftingtable & \mcwoodenpickaxe & \mcstonepickaxe & \mcironpickaxe & \mcdiamond \\
    \midrule
    DreamerV3 & - & 50.0 & 3.0 & 0.01 & 0.01 \\
    DEPS & 90.0 & 80.0 & 73.3 & 10.0 & 0.6\\
    VPT & 100.0 & 100.0 & 100.0 & 85.0 & 20.0\\
    Our GMIT & 100.0 & 100.0 & 100.0 & 95.0 & 67.5 \\
    \bottomrule
    \end{tabular}
    \label{tab:main_result}
\end{table}
